Enabling Research through the SCIP Optimization Suite 8.0

The SCIP Optimization Suite provides a collection of software packages for mathematical optimization centered around the constraint integer programming framework SCIP. The focus of this paper is on the role of the SCIP Optimization Suite in supporting research. SCIP's main design principles are discussed, followed by a presentation of the latest performance improvements and developments in version 8.0, which serve both as examples of SCIP's application as a research tool and as a platform for further developments. Further, the paper gives an overview of interfaces to other programming and modeling languages, new features that expand the possibilities for user interaction with the framework, and the latest developments in several extensions built upon SCIP.

==> section_core_benders.tex <==
\subsection{Benders' Decomposition}
\label{subsect:benders}

The most important update for the Benders' decomposition framework is the option to apply the mixed integer rounding (MIR) procedure, as described by Achterberg~\cite{Achterberg2007a}, when generating optimality cuts.
The aim of applying the MIR procedure to the generated optimality cut is to potentially compute a stronger inequality.


==> section_core_cutsel.tex <==
\subsection{Cut Selectors}
\label{subsect:cutselectors}

The new cut selector plugin is introduced in SCIP 8.0. Users now have the ability to create their own cut selection rules and include them into SCIP.
The ability to include cut selectors has also been implemented through PySCIPOpt.

